Deep Keypoint-Based Camera Pose Estimation with Geometric Constraints

Estimating relative camera poses from consecutive frames is a fundamental problem in visual odometry (VO) and simultaneous localization and mapping (SLAM), where classic methods consisting of hand-crafted features and sampling-based outlier rejection have been a dominant choice for over a decade. Although multiple works propose to replace these modules with learning-based counterparts, most have not yet been as accurate, robust and generalizable as conventional methods. In this paper, we design an end-to-end trainable framework consisting of learnable modules for detection, feature extraction, matching and outlier rejection, while directly optimizing for the geometric pose objective. We show both quantitatively and qualitatively that pose estimation performance may be achieved on par with the classic pipeline. Moreover, we are able to show by end-to-end training, the key components of the pipeline could be significantly improved, which leads to better generalizability to unseen datasets compared to existing learning-based methods.

==> sections/ablation.tex <==
\section{Ablation Study} \label{Ablation}


==> sections/notation.tex <==
%=============================================
\section{Notation} \label{Preliminaries}
We refer to the pair of images as $I, I' \in \mathbb{R}^{H\times W}$. 
The transformation matrix from frame $i$ to $j$ as $T_{ij} = [R| t]$, where $R \in \mathbb{R}^{3 \times 3}$ is the rotation matrix and $t \in \mathbb{R}^{3 \times 1}$ is the translation vector.
We refer to the point on 2d images as $p \in \mathbb{R}^2$, where $p = [u, v]$ denotes the $x, y$ coordinates of the point. 
% \subsection{Fundamental matrix from correspondences}
% \begin{equation} \label{eq_Fund}
%     minimized least squared 
% \end{equation}
% The equantion shows how we get fundamental matrix by minimizing least squared terms. We apply SVD.
% Residuals.

% Pose from F matrix. Chirarty check. 

==> tables/exp_ablation_apolloModels.tex <==
%%%% kitti model (main table) on kitti and apollo
\begin{table*}[h]
    \scriptsize
    \centering
    \begin{tabular}{lllllllllllll}
        \toprule
        \multirow{2}{*} {Apollo Models} & \multicolumn{6}{c}{KITTI dataset - error(deg.) inlier ratio$\uparrow$, mean$\downarrow$, median$\downarrow$} & \multicolumn{6}{c}{Apollo dataset} \\
        \cmidrule(r){2-7} \cmidrule(r){8-13}
        {}                               & \multicolumn{3}{c}{Rotation (deg.)} & \multicolumn{3}{c}{Translation (deg.)} & \multicolumn{3}{c}{Rotation} & \multicolumn{3}{c}{Translation} \\
         {} & 0.1$\uparrow$  & Mean.$\downarrow$ & Med.$\downarrow$ & 2.0$\uparrow$ & Mean.$\downarrow$ & Med.$\downarrow$ & 0.1 $\uparrow$ & Mean.$\downarrow$ & Med.$\downarrow$ & 2.0 $\uparrow$ & Mean.$\downarrow$ & Med.$\downarrow$ \\
        \midrule

% Si-Ran & \textbf{0.816} & 0.456 & 0.057 & 0.900 & 2.061 & 0.613 & 0.922 & 0.151 & 0.036 & 0.978 & 0.878 & 0.385
% \\ \hline
% Sp-Ran & 0.121 & 0.935 & 0.291 & 0.378 & 7.607 & 2.736 & 0.337 & 0.225 & 0.133 & 0.491 & 5.249 & 2.041
% \\ \hline
% Si-Df-f & 0.755 & 0.125 & 0.057 & 0.832 & 2.600 & 0.660 & 0.952 & 0.076 & 0.029 & 0.991 & 0.452 & 0.190
% \\ \hline
% Si-Df-p & 0.652 & 0.156 & 0.071 & 0.838 & 2.457 & 0.693 & 0.932 & 0.092 & 0.033 & 0.980 & 0.664 & 0.226
% \\ \hline
% Si-Df-fp & 0.747 & 0.112 & 0.057 & 0.824 & 2.267 & 0.692 & 0.952 & 0.062 & 0.028 & 0.993 & 0.343 & 0.144
% \\ \hline
% Sp-Df-f & 0.354 & 0.204 & 0.133 & 0.621 & 3.337 & 1.537 & 0.877 & 0.087 & 0.049 & 0.951 & 0.922 & 0.535
% \\ \hline
% Sp-Df-p & 0.268 & 0.229 & 0.161 & 0.609 & 3.749 & 1.577 & 0.893 & 0.088 & 0.046 & 0.973 & 0.763 & 0.434
% \\ \hline
% Sp-Df-f-end & 0.305 & 0.214 & 0.149 & 0.601 & 3.073 & 1.548 & 0.889 & 0.089 & 0.046 & 0.964 & 0.752 & 0.457
% \\ \hline
% Sp-Df-p-end & 0.235 & 0.275 & 0.186 & 0.557 & 3.740 & 1.712 & 0.226 & 0.273 & 0.187 & 0.551 & 3.457 & 1.756
% \\ \hline
% Sp-Df-fp-end & 0.373 & 0.174 & 0.128 & 0.674 & 2.496 & 1.318 & 0.915 & 0.067 & 0.043 & 0.983 & 0.669 & 0.367
% \\ \hline

Si-Ran & \textbf{ 0.816 } & 0.456 & \textbf{ 0.057 } & \textbf{ 0.900 } & \textbf{ 2.061 } & \textbf{ 0.613 } & 0.922 & 0.151 & 0.036 & 0.978 & 0.878 & 0.385
\\ \hline
Sp-Ran & 0.121 & 0.935 & 0.291 & 0.378 & 7.607 & 2.736 & 0.337 & 0.225 & 0.133 & 0.491 & 5.249 & 2.041
\\ \hline
Si-Df-f & \textbf{ 0.755 } & \textbf{ 0.125 } & 0.057 & 0.832 & 2.600 & \textbf{ 0.660 } & \textbf{ 0.952 } & 0.076 & \textbf{ 0.029 } & \textbf{ 0.991 } & \textbf{ 0.452 } & \textbf{ 0.190 }
\\ \hline
Si-Df-p & 0.652 & 0.156 & 0.071 & \textbf{ 0.838 } & 2.457 & 0.693 & 0.932 & 0.092 & 0.033 & 0.980 & 0.664 & 0.226
\\ \hline
Si-Df-fp & 0.747 & \textbf{ 0.112 } & \textbf{ 0.057 } & 0.824 & \textbf{ 2.267 } & 0.692 & \textbf{ 0.952 } & \textbf{ 0.062 } & \textbf{ 0.028 } & \textbf{ 0.993 } & \textbf{ 0.343 } & \textbf{ 0.144 }
\\ \hline
Sp-Df-f & 0.354 & 0.204 & 0.133 & 0.621 & 3.337 & 1.537 & 0.877 & 0.087 & 0.049 & 0.951 & 0.922 & 0.535
\\ \hline
Sp-Df-p & 0.268 & 0.229 & 0.161 & 0.609 & 3.749 & 1.577 & 0.893 & 0.088 & 0.046 & 0.973 & 0.763 & 0.434
\\ \hline
Sp-Df-f-end & 0.305 & 0.214 & 0.149 & 0.601 & 3.073 & 1.548 & 0.889 & 0.089 & 0.046 & 0.964 & 0.752 & 0.457
\\ \hline
% Sp-Df-p-end & 0.235 & 0.275 & 0.186 & 0.557 & 3.740 & 1.712 & 0.226 & 0.273 & 0.187 & 0.551 & 3.457 & 1.756
% \\ \hline
Sp-Df-p-end & 0.166 & 0.393 & 0.229 & 0.492 & 4.181 & 2.046 & 0.902 & 0.088 & 0.044 & 0.980 & 0.761 & 0.385
\\ \hline
Sp-Df-fp-end & 0.373 & 0.174 & 0.128 & 0.674 & 2.496 & 1.318 & 0.915 & \textbf{ 0.067 } & 0.043 & 0.983 & 0.669 & 0.367
\\ \hline

coco-Sp-Df-f & 0.218 & 0.206 & 0.171 & 0.538 & 3.196 & 1.850 & 0.877 & 0.087 & 0.049 & 0.951 & 0.922 & 0.535
\\ \hline
coco-Sp-Df-f-end & 0.256 & 0.227 & 0.170 & 0.582 & 3.452 & 1.684 & 0.889 & 0.089 & 0.046 & 0.964 & 0.752 & 0.457
\\ \hline

\bottomrule
    \end{tabular}
\caption{\label{tab:exp_ablation_apolloModels} \textbf{Apollo model on KITTI and Apollo dataset. The main table for rotation and translation error.} The set of models are trained in solely in KITTI dataset or ApolloScape dataset. }
\end{table*}

==> tables/exp_ablation_kittiModels.tex <==
%%%% kitti model (main table) on kitti and apollo
\begin{table*}[h]
    \scriptsize
    \centering
    \begin{tabular}{lllllllllllll}
        \toprule
        \multirow{2}{*} {KITTI Models} & \multicolumn{6}{c}{KITTI dataset - error(deg.) inlier ratio$\uparrow$, mean$\downarrow$, median$\downarrow$} & \multicolumn{6}{c}{Apollo dataset} \\
        \cmidrule(r){2-7} \cmidrule(r){8-13}
        {}                               & \multicolumn{3}{c}{Rotation (deg.)} & \multicolumn{3}{c}{Translation (deg.)} & \multicolumn{3}{c}{Rotation} & \multicolumn{3}{c}{Translation} \\
         {} & 0.1$\uparrow$  & Mean.$\downarrow$ & Med.$\downarrow$ & 2.0$\uparrow$ & Mean.$\downarrow$ & Med.$\downarrow$ & 0.1 $\uparrow$ & Mean.$\downarrow$ & Med.$\downarrow$ & 2.0 $\uparrow$ & Mean.$\downarrow$ & Med.$\downarrow$ \\
        \midrule


Si-Ran & 0.818 & 0.391 & 0.056 & 0.899 & 1.895 & 0.639 & \textbf{0.922} & 0.157 & \textbf{0.037} & \textbf{0.979} & \textbf{0.788} & \textbf{0.388}
\\ \hline
Sp-Ran & 0.189 & 0.641 & 0.217 & 0.481 & 5.798 & 2.103 & 0.407 & 0.205 & 0.118 & 0.583 & 5.645 & 1.670
\\ \hline
Si-Df-f & \textbf{0.938} & \textbf{0.051} & \textbf{0.041} & 0.914 & 1.699 & \textbf{0.484} & 0.845 & 0.172 & \textbf{0.043} & 0.895 & 2.452 & 0.389
\\ \hline
Si-Df-p & 0.901 & 0.059 & 0.044 & 0.903 & \textbf{1.472} & 0.513 & 0.727 & 0.333 & 0.056 & 0.760 & 4.918 & 0.658
\\ \hline
Si-Df-fp & \textbf{0.947} & 0.111 & \textbf{0.038} & \textbf{0.916} & 1.741 & \textbf{0.484} & 0.840 & 0.148 & 0.044 & 0.911 & 2.103 & \textbf{0.369}
\\ \hline
Sp-Df-f & 0.633 & 0.100 & 0.078 & 0.830 & 1.476 & 0.846 & 0.725 & 0.126 & 0.068 & 0.754 & 2.074 & 1.155
\\ \hline
Sp-Df-p & 0.875 & 0.130 & 0.047 & 0.887 & 1.719 & 0.539 & 0.730 & 0.124 & 0.067 & 0.827 & 1.905 & 0.974
\\ \hline
Sp-Df-f-end & 0.915 & 0.053 & 0.042 & 0.905 & 1.662 & 0.489 & 0.841 & \textbf{0.100} & 0.051 & 0.910 & \textbf{1.122} & 0.589
\\ \hline
Sp-Df-p-end & 0.932 & \textbf{0.050} & 0.041 & 0.905 & 1.600 & 0.503 & 0.686 & 0.152 & 0.071 & 0.747 & 2.652 & 1.068
\\ \hline
Sp-Df-fp-end & 0.910 & 0.054 & 0.048 & \textbf{0.917} & \textbf{1.062} & 0.504 & \textbf{0.864} & \textbf{0.092} & 0.051 & \textbf{0.924} & 1.275 & 0.659
\\ \hline


% Si-Ran & 0.818 & 0.391 & 0.056 & 0.899 & 1.895 & 0.639 & 0.922 & 0.157 & 0.037 & 0.979 & 0.788 & 0.388
% \\ \hline
% Sp-Ran & 0.189 & 0.641 & 0.217 & 0.481 & 5.798 & 2.103 & 0.407 & 0.205 & 0.118 & 0.583 & 5.645 & 1.670
% \\ \hline
% Si-Df-f & 0.938 & 0.051 & 0.041 & 0.914 & 1.699 & 0.484 & 0.845 & 0.172 & 0.043 & 0.895 & 2.452 & 0.389
% \\ \hline
% Si-Df-p & 0.901 & 0.059 & 0.044 & 0.903 & 1.472 & 0.513 & 0.727 & 0.333 & 0.056 & 0.760 & 4.918 & 0.658
% \\ \hline
% Si-Df-fp & 0.947 & 0.111 & 0.038 & 0.916 & 1.741 & 0.484 & 0.840 & 0.148 & 0.044 & 0.911 & 2.103 & 0.369
% \\ \hline
% Sp-Df-f & 0.633 & 0.100 & 0.078 & 0.830 & 1.476 & 0.846 & 0.725 & 0.126 & 0.068 & 0.754 & 2.074 & 1.155
% \\ \hline
% Sp-Df-p & 0.875 & 0.130 & 0.047 & 0.887 & 1.719 & 0.539 & 0.730 & 0.124 & 0.067 & 0.827 & 1.905 & 0.974
% \\ \hline
% Sp-Df-f-end & 0.915 & 0.053 & 0.042 & 0.905 & 1.662 & 0.489 & 0.841 & 0.100 & 0.051 & 0.910 & 1.122 & 0.589
% \\ \hline
% Sp-Df-p-end & 0.932 & 0.050 & 0.041 & 0.905 & 1.600 & 0.503 & 0.686 & 0.152 & 0.071 & 0.747 & 2.652 & 1.068
% \\ \hline
% Sp-Df-fp-end & 0.910 & 0.054 & 0.048 & 0.917 & 1.062 & 0.504 & 0.864 & 0.092 & 0.051 & 0.924 & 1.275 & 0.659
% \\ \hline


\bottomrule
    \end{tabular}
\caption{\label{tab:exp_ablation_kittiModels} \textbf{KITTI model on Apollo dataset. The full table for rotation and translation error.} The set of models are trained in solely in KITTI dataset or ApolloScape dataset. }
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \scriptsize
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{} {\multirow{2}{*}{Models (KITTI)}} & \multicolumn{8}{l|}{KITTI dataset - Inlier ratio (w/i i degree)}       \\ \cline{2-9} 
%                   {}                                & \multicolumn{4}{l|}{Rot.} & \multicolumn{4}{l|}{Trans} \\ \cline{2-9} 
%                   & 0.02 & 0.1   & 1     & med.  & 0.1   & 1 & 2     & med.        \\ \hline
% {[}0{]}            & &&&&&&&                     \\ \hline
% {[}1{]}            & 0.007 & 0.252 & 0.966 & 0.177 & 0.003 & 0.234 & 0.483 & 2.050                     \\ \hline
% {[}2{]}            & 0.126 & 0.942 & 0.999 & 0.043 & 0.022 & 0.751 & 0.857 & 0.562   \\ \hline
% {[}3{]}            & 0.105 & 0.882 & 0.996 & 0.047 & 0.014 & 0.717 & 0.833 & 0.603 \\ \hline
% {[}4{]}            & 0.144 & 0.939 & 1.000 & 0.042 & 0.022 & 0.737 & 0.850 & 0.567 \\ \hline
% {[}5{]}            & 0.007 & 0.435 & 0.999 & 0.112 & 0.007 & 0.428 & 0.668 & 1.187 \\ \hline
% {[}6{]}            & 0.033 & 0.647 & 0.998 & 0.078 & 0.012 & 0.547 & 0.766 & 0.898 \\ \hline
% {[}7{]}            & 0.107 & 0.872 & 1.000 & 0.051 & 0.018 & 0.729 & 0.843 & 0.598 \\ \hline
% {[}8{]}            & 0.091 & 0.772 & 0.998 & 0.060 & 0.027 & 0.680 & 0.831 & 0.685 \\ \hline
% {[}9{]}            & 0.103 & 0.910 & 1.000 & 0.048 & 0.037 & 0.805 & 0.917 & 0.504   \\ \hline
% \end{tabular}
% \caption{\label{tab:exp_ablation_pipe} \textbf{Ablation study.} }
% \end{table*}


==> tables/supp_ablation_apolloModels.tex <==
%%%%% apollo model on apollo
\begin{table*}[h]
    \scriptsize
    \centering
    \begin{tabular}{lllllllllllllll}
        \toprule
        \multirow{2}{*} {Apollo dataset} & \multicolumn{7}{c}{Rotation (inlier ratio, error median)} & \multicolumn{7}{c}{Translation (inlier ratio, error median)} \\
        \cmidrule(r){2-8} \cmidrule(r){9-15} \\
         Apollo Models & 0.01 & 0.02 & 0.05 & 0.1 & 0.5 & Mean & Med. & 0.1 & 0.2 & 0.5 & 1.0 & 2.0 & Mean & Med. \\
        \midrule
  
Base(Si-Ran) & 0.058 & 0.227 & 0.662 & 0.922 & 0.997 & 0.157 & 0.037 & 0.065 & 0.214 & 0.623 & 0.890 & 0.979 & 0.788 & 0.388
\\ \hline
Base(Sp-Ran) & 0.000 & 0.007 & 0.090 & 0.355 & 0.952 & 0.202 & 0.128 & 0.003 & 0.011 & 0.061 & 0.213 & 0.524 & 4.816 & 1.899
\\ \hline
Si-Df-f & 0.069 & 0.239 & 0.670 & 0.912 & 0.997 & 0.079 & 0.036 & 0.126 & 0.338 & 0.719 & 0.884 & 0.954 & 0.745 & 0.293
\\ \hline
Si-Df-p & 0.110 & 0.308 & 0.729 & 0.942 & 0.997 & 0.097 & 0.031 & 0.216 & 0.506 & 0.850 & 0.953 & 0.987 & 0.455 & 0.197
\\ \hline
Sp-Df-f & 0.013 & 0.078 & 0.483 & 0.860 & 0.996 & 0.096 & 0.051 & 0.027 & 0.099 & 0.428 & 0.784 & 0.944 & 0.972 & 0.573
\\ \hline
Sp-Df-p & 0.014 & 0.088 & 0.499 & 0.865 & 0.997 & 0.094 & 0.050 & 0.041 & 0.139 & 0.520 & 0.836 & 0.961 & 0.855 & 0.483
\\ \hline
Ours(Sp-Df-f-end) & 0.012 & 0.098 & 0.553 & 0.900 & 0.999 & 0.086 & 0.046 & 0.044 & 0.144 & 0.560 & 0.876 & 0.970 & 0.769 & 0.451
\\ \hline
Ours(Sp-Df-p-end) & 0.018 & 0.107 & 0.580 & 0.905 & 0.998 & 0.085 & 0.044 & 0.047 & 0.178 & 0.637 & 0.903 & 0.975 & 0.708 & 0.398
\\ \hline
Ours(Sp-Df-fp-end) & 0.020 & 0.117 & 0.593 & 0.910 & 0.999 & 0.084 & 0.043 & 0.042 & 0.149 & 0.555 & 0.881 & 0.977 & 0.714 & 0.454
\\ \hline

Sp-D-a-p-b16 & 0.012 & 0.077 & 0.496 & 0.865 & 0.998 & 0.091 & 0.050 & 0.034 & 0.124 & 0.502 & 0.850 & 0.964 & 1.052 & 0.497
\\ \hline

Si-D-a-p-b4 & 0.061 & 0.215 & 0.623 & 0.888 & 0.995 & 0.122 & 0.039 & 0.093 & 0.283 & 0.634 & 0.831 & 0.931 & 0.936 & 0.353
\\ \hline
Sp-D-end-a-p-b12 & 0.020 & 0.111 & 0.565 & 0.900 & 0.999 & 0.086 & 0.046 & 0.049 & 0.172 & 0.599 & 0.896 & 0.977 & 0.805 & 0.421
\\ \hline

Sp-D-f-b12 & 0.012 & 0.088 & 0.508 & 0.876 & 0.999 & 0.089 & 0.049 & 0.037 & 0.130 & 0.489 & 0.828 & 0.962 & 1.050 & 0.509
\\ \hline
Sp-D-f-end-b8 & 0.021 & 0.124 & 0.592 & 0.914 & 0.999 & 0.084 & 0.044 & 0.044 & 0.154 & 0.576 & 0.884 & 0.976 & 0.774 & 0.443
\\ \hline

% Si-Ran & 0.054 & 0.226 & 0.662 & 0.922 & 0.996 & 0.151 & 0.036 & 0.066 & 0.220 & 0.629 & 0.895 & 0.978 & 0.878 & 0.385
% \\ \hline
% Sp-Ran & 0.001 & 0.007 & 0.074 & 0.337 & 0.951 & 0.225 & 0.133 & 0.003 & 0.010 & 0.061 & 0.201 & 0.491 & 5.249 & 2.041
% \\ \hline
% Si-Df-f & 0.108 & 0.323 & 0.751 & 0.952 & 0.997 & 0.076 & 0.029 & 0.217 & 0.526 & 0.889 & 0.974 & 0.991 & 0.452 & 0.190
% \\ \hline
% Si-Df-p & 0.085 & 0.274 & 0.707 & 0.932 & 0.994 & 0.092 & 0.033 & 0.171 & 0.441 & 0.810 & 0.940 & 0.980 & 0.664 & 0.226
% \\ \hline
% Si-Df-fp & 0.133 & 0.350 & 0.765 & 0.952 & 0.998 & 0.062 & 0.028 & 0.324 & 0.672 & 0.946 & 0.985 & 0.993 & 0.343 & 0.144
% \\ \hline
% Sp-Df-f & 0.013 & 0.091 & 0.509 & 0.877 & 0.997 & 0.087 & 0.049 & 0.027 & 0.106 & 0.462 & 0.803 & 0.951 & 0.922 & 0.535
% \\ \hline
% Sp-Df-p & 0.013 & 0.105 & 0.554 & 0.893 & 0.997 & 0.088 & 0.046 & 0.042 & 0.155 & 0.587 & 0.888 & 0.973 & 0.763 & 0.434
% \\ \hline
% Sp-Df-f-end & 0.014 & 0.100 & 0.553 & 0.889 & 0.998 & 0.089 & 0.046 & 0.038 & 0.135 & 0.550 & 0.866 & 0.964 & 0.752 & 0.457
% \\ \hline
% % Sp-Df-p-end & 0.001 & 0.006 & 0.051 & 0.226 & 0.888 & 0.273 & 0.187 & 0.004 & 0.018 & 0.087 & 0.276 & 0.551 & 3.457 & 1.756
% % \\ \hline
% Sp-Df-p-end & 0.018 & 0.109 & 0.575 & 0.902 & 0.998 & 0.088 & 0.044 & 0.053 & 0.190 & 0.651 & 0.917 & 0.980 & 0.761 & 0.385
% \\ \hline
% Sp-Df-fp-end & 0.017 & 0.125 & 0.592 & 0.915 & 0.999 & 0.067 & 0.043 & 0.058 & 0.206 & 0.676 & 0.931 & 0.983 & 0.669 & 0.367
% \\ \hline

\bottomrule
    \end{tabular}
\caption{\label{tab:exp_ablation_ref_table} \textbf{Apollo model on Apollo dataset. The full table for rotation and translation error.} The set of models are trained in solely in KITTI dataset or ApolloScape dataset. }
\end{table*}

%%%% apollo models on kitti
\begin{table*}[h]
    \scriptsize
    \centering
    \begin{tabular}{lllllllllllllll}
        \toprule
        \multirow{2}{*} {Apollo dataset} & \multicolumn{7}{c}{Rotation (inlier ratio, error median)} & \multicolumn{7}{c}{Translation (inlier ratio, error median)} \\
        \cmidrule(r){2-8} \cmidrule(r){9-15} \\
         Apollo Models & 0.01 & 0.02 & 0.05 & 0.1 & 0.5 & Mean & Med. & 0.1 & 0.2 & 0.5 & 1.0 & 2.0 & Mean & Med. \\
        \midrule
Base(Si-Ran) & 0.011 & 0.068 & 0.427 & 0.816 & 0.997 & 0.456 & 0.057 & 0.024 & 0.084 & 0.390 & 0.735 & 0.900 & 1.980 & 0.613
\\ \hline
Base(Sp-Ran) & 0.000 & 0.006 & 0.031 & 0.102 & 0.627 & 1.178 & 0.367 & 0.001 & 0.005 & 0.033 & 0.114 & 0.304 & 11.085 & 3.330
\\ \hline
Si-Df-f & 0.010 & 0.056 & 0.365 & 0.706 & 0.964 & 0.130 & 0.066 & 0.022 & 0.074 & 0.362 & 0.663 & 0.824 & 3.133 & 0.686
\\ \hline
Si-Df-p & 0.015 & 0.091 & 0.449 & 0.786 & 0.980 & 0.096 & 0.054 & 0.018 & 0.075 & 0.392 & 0.725 & 0.860 & 1.932 & 0.606
\\ \hline
Sp-Df-f & 0.000 & 0.003 & 0.029 & 0.124 & 0.693 & 0.426 & 0.313 & 0.001 & 0.006 & 0.033 & 0.122 & 0.308 & 4.695 & 3.365
\\ \hline
Sp-Df-p & 0.000 & 0.003 & 0.028 & 0.113 & 0.718 & 0.413 & 0.311 & 0.001 & 0.005 & 0.032 & 0.116 & 0.303 & 5.227 & 3.509
\\ \hline
Ours(Sp-Df-f-end) & 0.001 & 0.008 & 0.059 & 0.217 & 0.904 & 0.248 & 0.194 & 0.000 & 0.006 & 0.057 & 0.231 & 0.510 & 3.070 & 1.954
\\ \hline
Ours(Sp-Df-p-end) & 0.001 & 0.008 & 0.064 & 0.279 & 0.960 & 0.198 & 0.161 & 0.005 & 0.013 & 0.089 & 0.309 & 0.617 & 2.614 & 1.554
\\ \hline
Ours(Sp-Df-fp-end) & 0.003 & 0.012 & 0.110 & 0.353 & 0.962 & 0.177 & 0.132 & 0.004 & 0.013 & 0.086 & 0.328 & 0.649 & 2.352 & 1.435
\\ \hline

Sp-D-a-p-b16 & 0.002 & 0.013 & 0.138 & 0.424 & 0.956 & 0.170 & 0.118 & 0.007 & 0.028 & 0.149 & 0.422 & 0.699 & 2.442 & 1.190
\\ \hline

Si-D-a-p-b4 & 0.012 & 0.067 & 0.347 & 0.667 & 0.946 & 0.154 & 0.069 & 0.017 & 0.071 & 0.303 & 0.597 & 0.773 & 2.795 & 0.779
\\ \hline
Sp-D-end-a-p-b12 & 0.004 & 0.019 & 0.169 & 0.467 & 0.973 & 0.159 & 0.106 & 0.006 & 0.025 & 0.152 & 0.443 & 0.750 & 2.466 & 1.112
\\ \hline
Sp-D-f-b12 & 0.001 & 0.017 & 0.151 & 0.454 & 0.957 & 0.173 & 0.110 & 0.008 & 0.028 & 0.147 & 0.406 & 0.684 & 3.068 & 1.239
\\ \hline
Sp-D-f-end-b8 & 0.004 & 0.021 & 0.185 & 0.529 & 0.978 & 0.135 & 0.094 & 0.006 & 0.029 & 0.182 & 0.485 & 0.767 & 2.454 & 1.032
\\ \hline
        
% Si-Ran & 0.011 & 0.068 & 0.427 & 0.816 & 0.997 & 0.456 & 0.057 & 0.024 & 0.083 & 0.390 & 0.735 & 0.900 & 2.061 & 0.613
% \\ \hline
% Sp-Ran & 0.000 & 0.003 & 0.027 & 0.121 & 0.719 & 0.935 & 0.291 & 0.001 & 0.007 & 0.046 & 0.152 & 0.378 & 7.607 & 2.736
% \\ \hline
% Si-Df-f & 0.011 & 0.078 & 0.435 & 0.755 & 0.960 & 0.125 & 0.057 & 0.018 & 0.072 & 0.352 & 0.683 & 0.832 & 2.600 & 0.660
% \\ \hline
% Si-Df-p & 0.011 & 0.057 & 0.336 & 0.652 & 0.954 & 0.156 & 0.071 & 0.013 & 0.068 & 0.313 & 0.663 & 0.838 & 2.457 & 0.693
% \\ \hline
% Si-Df-fp & 0.016 & 0.085 & 0.439 & 0.747 & 0.970 & 0.112 & 0.057 & 0.019 & 0.078 & 0.339 & 0.673 & 0.824 & 2.267 & 0.692
% \\ \hline
% Sp-Df-f & 0.001 & 0.010 & 0.095 & 0.354 & 0.952 & 0.204 & 0.133 & 0.004 & 0.014 & 0.098 & 0.314 & 0.621 & 3.337 & 1.537
% \\ \hline
% Sp-Df-p & 0.000 & 0.006 & 0.062 & 0.268 & 0.925 & 0.229 & 0.161 & 0.005 & 0.015 & 0.100 & 0.296 & 0.609 & 3.749 & 1.577
% \\ \hline
(old)Sp-Df-f-end & 0.001 & 0.009 & 0.087 & 0.305 & 0.932 & 0.214 & 0.149 & 0.003 & 0.014 & 0.097 & 0.314 & 0.601 & 3.073 & 1.548
\\ \hline

% Sp-Df-p-end & 0.001 & 0.003 & 0.055 & 0.235 & 0.891 & 0.275 & 0.186 & 0.004 & 0.014 & 0.089 & 0.268 & 0.557 & 3.740 & 1.712
% \\ \hline
(old)Sp-Df-p-end & 0.000 & 0.004 & 0.030 & 0.166 & 0.833 & 0.393 & 0.229 & 0.002 & 0.007 & 0.060 & 0.207 & 0.492 & 4.181 & 2.046
\\ \hline
(old)Sp-Df-fp-end & 0.001 & 0.008 & 0.104 & 0.373 & 0.967 & 0.174 & 0.128 & 0.004 & 0.019 & 0.112 & 0.371 & 0.674 & 2.496 & 1.318
\\ \hline

\bottomrule
    \end{tabular}
\caption{\label{tab:exp_ablation_ref_table} \textbf{Apollo model on KITTI dataset. The full table for rotation and translation error.} The set of models are trained in solely in KITTI dataset or ApolloScape dataset. }
\end{table*}




==> tables/supp_ablation_apolloModels_smallTables.tex <==
%%%% Apollo model (small tables) 


%%%% Apollo models - ours on apollo
% table: table_apolloModels_our_apo
\begin{table}[h]
    \scriptsize
    \centering
    \begin{tabular}{lllllll}
        \toprule
        \multirow{2}{*} {Apollo Models} & \multicolumn{6}{c}{Apollo dataset - error(deg.) inlier ratio$\uparrow$, mean$\downarrow$, median$\downarrow$}  \\
        \cmidrule(r){2-7}
        {}                               & \multicolumn{3}{c}{Rotation (deg.)} & \multicolumn{3}{c}{Translation (deg.)} \\
         {} & 0.1$\uparrow$  & Mean.$\downarrow$ & Med.$\downarrow$ & 2.0$\uparrow$ & Mean.$\downarrow$ & Med.$\downarrow$ \\
        \midrule

Base(Sp-Ran) & 0.320 & 0.271 & 0.138 & 0.489 & 5.887 & 2.044
\\ \hline
Sp-Df-f & 0.876 & 0.089 & 0.049 & 0.962 & 1.050 & 0.509
\\ \hline
Sp-Df-p & 0.865 & 0.091 & 0.050 & 0.964 & 1.052 & 0.497
\\ \hline
Ours(Sp-Df-f-end) & 0.914 & 0.084 & 0.044 & 0.976 & \textbf{0.774} & 0.443
\\ \hline
Ours(Sp-Df-p-end) & 0.900 & 0.086 & 0.046 & 0.977 & 0.805 & 0.421
\\ \hline
Ours(Sp-Df-fp-end) & \textbf{0.921} & \textbf{0.082} & \textbf{0.042} & \textbf{0.977} & 0.903 & \textbf{0.406}
\\ \hline

\bottomrule
    \end{tabular}
\caption{\label{tab:exp_ablation_apollo-apo-ours} \textbf{Comparison of pose estimation for our Apollo models on Apollo dataset.} 
The set of models are trained in Apollo dataset with learning-based feature extraction (FE). It shows improvement from RANSAC to DeepF pose estimation, and the benefits from separate models to end-to-end training. The end-to-end model shows the best mean and median errors.
}
% The table compares the learning based approaches in a cross dataset setting. The table shows that our end-to-end \texttt{DeepFEPE} performs the best.
\end{table}


%%%% Apollo models - baseline on apollo
% table: table_apolloModels_baselines_apo
\begin{table}[h]
    \scriptsize
    \centering
    \begin{tabular}{lllllll}
        \toprule
        \multirow{2}{*} {KITTI Models} & \multicolumn{6}{c}{Apollo dataset - error(deg.) inlier ratio$\uparrow$, mean$\downarrow$, median$\downarrow$}  \\
        \cmidrule(r){2-7}
        {}                               & \multicolumn{3}{c}{Rotation (deg.)} & \multicolumn{3}{c}{Translation (deg.)} \\
         {} & 0.1$\uparrow$  & Mean.$\downarrow$ & Med.$\downarrow$ & 2.0$\uparrow$ & Mean.$\downarrow$ & Med.$\downarrow$ \\
        \midrule

Base(Si-Ran) & 0.922 & 0.157 & 0.037 & 0.979 & 0.788 & 0.388
\\ \hline
Si-Df-f & 0.912 & \textbf{0.079} & 0.036 & 0.954 & 0.745 & 0.293
\\ \hline
Si-Df-p & \textbf{0.942} & 0.097 & \textbf{0.031} & \textbf{0.987} & \textbf{0.455} & \textbf{0.197}
\\ \hline
Ours(Sp-Df-fp-end) & 0.921 & 0.082 & 0.042 & 0.977 & 0.903 & 0.406
\\ \hline


\bottomrule
    \end{tabular}
\caption{\label{tab:exp_ablation_apollo-apo-base} \textbf{Comparison of pose estimation for Baseline Apollo models on Apollo dataset.} 
The table compares our best \texttt{DeepFEPE} model with SIFT based pose estimation. Our model performs on par with classic pipeline. The SIFT+DeepF pipeline is boosted with our geometry-based pose loss.
}
% The table compares our \texttt{DeepFEPE} with other baseline methods in a cross dataset setting. The results show that traditional method (SIFT + RANSAC) maintains the best overall results. Our model performs better than Si-models.
\end{table}

%%%% ours - kitti
% table: table_apolloModels_ours_kit
\begin{table}[h]
    \scriptsize
    \centering
    \begin{tabular}{lllllll}
        \toprule
        \multirow{2}{*} {Apollo Models} & \multicolumn{6}{c}{KITTI dataset - error(deg.) inlier ratio$\uparrow$, mean$\downarrow$, median$\downarrow$}  \\
        \cmidrule(r){2-7} 
        {}                               & \multicolumn{3}{c}{Rotation (deg.)} & \multicolumn{3}{c}{Translation (deg.)} \\
         {} & 0.1$\uparrow$  & Mean.$\downarrow$ & Med.$\downarrow$ & 2.0$\uparrow$ & Mean.$\downarrow$ & Med.$\downarrow$ \\
        \midrule
Base(Sp-Ran) & 0.190 & 0.820 & 0.224 & 0.472 & 7.142 & 2.162
\\ \hline
Sp-Df-f & 0.454 & 0.173 & 0.110 & 0.684 & 3.068 & 1.239
\\ \hline
Sp-Df-p & 0.424 & 0.170 & 0.118 & 0.699 & 2.442 & 1.190
\\ \hline
Ours(Sp-Df-f-end) & 0.529 & 0.135 & 0.094 & 0.767 & 2.454 & 1.032
\\ \hline
Ours(Sp-Df-p-end) & 0.467 & 0.159 & 0.106 & 0.750 & 2.466 & 1.112
\\ \hline
Ours(Sp-Df-fp-end) & \textbf{0.571} & \textbf{0.120} & \textbf{0.089} & \textbf{0.809} & \textbf{2.283} & \textbf{0.910}
\\ \hline

\bottomrule
    \end{tabular}
\caption{\label{tab:exp_ablation_apollo-kit-ours} \textbf{Comparison of pose estimation for learning-based Apollo models on KITTI dataset.} 
The table compares the learning-based models in a cross-dataset setting, which shows the clear gain from end-to-end training.
}
% The set of models are trained in KITTI with learning based feature extraction (FE). It shows significant improvement from RANSAC to DeepF pose estimation, and from separate models to end-to-end training.
\end{table}

%%%% baselines - kitti
% table: table_apolloModels_baselines_kit
\begin{table}[h]
    \scriptsize
    \centering
    \begin{tabular}{lllllll}
        \toprule
        \multirow{2}{*} {Apollo Models} & \multicolumn{6}{c}{KITTI dataset - error(deg.) inlier ratio$\uparrow$, mean$\downarrow$, median$\downarrow$}  \\
        \cmidrule(r){2-7} 
        {}                               & \multicolumn{3}{c}{Rotation (deg.)} & \multicolumn{3}{c}{Translation (deg.)} \\
         {} & 0.1$\uparrow$  & Mean.$\downarrow$ & Med.$\downarrow$ & 2.0$\uparrow$ & Mean.$\downarrow$ & Med.$\downarrow$ \\
        \midrule
Base(Si-Ran) & \textbf{0.818} & 0.391 & 0.056 & \textbf{0.899} & \textbf{1.895} & 0.639
\\ \hline
Si-Df-f & 0.706 & 0.130 & 0.066 & 0.824 & 3.133 & 0.686
\\ \hline
Si-Df-p & 0.786 & \textbf{0.096} & \textbf{0.054} & 0.860 & 1.932 & \textbf{0.606}
\\ \hline
Ours(Sp-Df-fp-end) & 0.571 & 0.120 & 0.089 & 0.809 & 2.283 & 0.910
\\ \hline

\bottomrule
    \end{tabular}
\caption{\label{tab:exp_ablation_apollo-kit-base} \textbf{Comparison of pose estimation for SIFT based Apollo models on KITTI dataset.} 
The table compares our best \texttt{DeepFEPE} model with SIFT based models.
}
% The table compare our best \texttt{DeepFEPE} model (End-to-end training with pose and F. loss) with SIFT based pose estimation. Our model works better than T-base, and comparable with state-of-the-art Si-models. 
\end{table}

==> tables/supp_ablation_kittiModels.tex <==
%%%%% kitti model on KITTI
\begin{table*}[h]
    \scriptsize
    \centering
    \begin{tabular}{llllllllllllllll}
        \toprule
        \multicolumn{2}{c}{\multirow{2}{*} {KITTI dataset}} & \multicolumn{7}{c}{Rotation (inlier ratio, error median)} & \multicolumn{7}{c}{Translation (inlier ratio, error median)} \\
        \cmidrule(r){3-9} \cmidrule(r){10-16} \\
        Catogories & KITTI Models & 0.01 & 0.02 & 0.05 & 0.1 & 0.5 & Mean & Med. & 0.1 & 0.2 & 0.5 & 1.0 & 2.0 & Mean & Med. \\
        \midrule

\textbf{Si-base} 
& Si-Ran & 0.017 & 0.078 & 0.433 & 0.818 & 0.997 & 0.391 & 0.056 & 0.020 & 0.085 & 0.372 & 0.727 & 0.899 & 1.895 & 0.639
\\ \midrule % \hline
\textbf{Sp-base} 
& Sp-Ran & 0.001 & 0.004 & 0.048 & 0.189 & 0.815 & 0.641 & 0.217 & 0.003 & 0.014 & 0.077 & 0.222 & 0.481 & 5.798 & 2.103
\\ \midrule % \hline
\textbf{Si-models} 
& Si-Df-f & 0.028 & 0.143 & 0.645 & 0.938 & 0.998 & 0.051 & 0.041 & 0.032 & 0.137 & 0.517 & 0.812 & 0.914 & 1.699 & 0.484
\\  % \hline
& Si-Df-p & 0.028 & 0.125 & 0.579 & 0.901 & 0.995 & 0.059 & 0.044 & 0.025 & 0.119 & 0.485 & 0.787 & 0.903 & 1.472 & 0.513
\\ % \hline
& Si-Df-fp & 0.028 & 0.161 & 0.680 & 0.947 & 0.998 & 0.111 & 0.038 & 0.037 & 0.135 & 0.519 & 0.816 & 0.916 & 1.741 & 0.484
\\ \midrule % \hline
\textbf{Sp-models} 
& Sp-Df-f & 0.005 & 0.034 & 0.263 & 0.633 & 0.997 & 0.100 & 0.078 & 0.009 & 0.048 & 0.258 & 0.579 & 0.830 & 1.476 & 0.846
\\ % \hline
& Sp-Df-p & 0.023 & 0.100 & 0.527 & 0.875 & 0.996 & 0.130 & 0.047 & 0.025 & 0.108 & 0.454 & 0.770 & 0.887 & 1.719 & 0.539
\\ \midrule % \hline
\texttt{DeepFEPE} 
& Sp-Df-f-end & 0.023 & 0.144 & 0.614 & 0.915 & 0.998 & 0.053 & 0.042 & 0.033 & 0.114 & 0.511 & 0.800 & 0.905 & 1.662 & 0.489
\\ 
& Sp-Df-p-end & 0.021 & 0.142 & 0.613 & 0.932 & 1.000 & 0.050 & 0.041 & 0.029 & 0.119 & 0.498 & 0.798 & 0.905 & 1.600 & 0.503
\\ 
& Sp-Df-fp-end & 0.018 & 0.103 & 0.535 & 0.910 & 1.000 & 0.054 & 0.048 & 0.037 & 0.131 & 0.498 & 0.805 & 0.917 & 1.062 & 0.504
\\ \hline

 \bottomrule % \hline
\end{tabular} 

\caption{\label{tab:exp_ablation_ref_table} \textbf{KITTI model on KITTI dataset. The full table for rotation and translation error.} The set of models are trained in solely in KITTI dataset or ApolloScape dataset. }
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% kitti model on apollo
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h]
    \scriptsize
    \centering
    \begin{tabular}{llllllllllllllll}
        \toprule
        \multicolumn{2}{c}{\multirow{2}{*} {Apollo dataset}} & \multicolumn{7}{c}{Rotation (inlier ratio, error median)} & \multicolumn{7}{c}{Translation (inlier ratio, error median)} \\
        \cmidrule(r){3-9} \cmidrule(r){10-16} \\
        Catogories & KITTI Models & 0.01 & 0.02 & 0.05 & 0.1 & 0.5 & Mean & Med. & 0.1 & 0.2 & 0.5 & 1.0 & 2.0 & Mean & Med. \\
        \midrule

\textbf{Si-base} 
& Si-Ran & 0.058 & 0.227 & 0.662 & 0.922 & 0.997 & 0.157 & 0.037 & 0.065 & 0.214 & 0.623 & 0.890 & 0.979 & 0.788 & 0.388
\\ \midrule % \hline
\textbf{Sp-base} 
& Sp-Ran & 0.001 & 0.012 & 0.114 & 0.407 & 0.962 & 0.205 & 0.118 & 0.003 & 0.016 & 0.089 & 0.271 & 0.583 & 5.645 & 1.670
\\ \midrule % \hline
\textbf{Si-models} 
& Si-Df-f & 0.043 & 0.187 & 0.567 & 0.845 & 0.963 & 0.172 & 0.043 & 0.093 & 0.246 & 0.593 & 0.791 & 0.895 & 2.452 & 0.389
\\  % \hline
& Si-Df-p & 0.035 & 0.132 & 0.451 & 0.727 & 0.904 & 0.333 & 0.056 & 0.053 & 0.156 & 0.425 & 0.614 & 0.760 & 4.918 & 0.658
\\ % \hline
& Si-Df-fp & 0.040 & 0.169 & 0.561 & 0.840 & 0.971 & 0.148 & 0.044 & 0.098 & 0.271 & 0.608 & 0.807 & 0.911 & 2.103 & 0.369
\\ \midrule % \hline
\textbf{Sp-models} 
& Sp-Df-f & 0.005 & 0.041 & 0.315 & 0.725 & 0.989 & 0.126 & 0.068 & 0.007 & 0.032 & 0.155 & 0.425 & 0.754 & 2.074 & 1.155
\\ % \hline
& Sp-Df-p & 0.004 & 0.040 & 0.329 & 0.730 & 0.989 & 0.124 & 0.067 & 0.009 & 0.036 & 0.192 & 0.513 & 0.827 & 1.905 & 0.974
\\ \midrule % \hline
\texttt{DeepFEPE} 
& Sp-Df-f-end  & 0.012 & 0.088 & 0.487 & 0.841 & 0.992 & 0.100 & 0.051 & 0.025 & 0.092 & 0.416 & 0.750 & 0.910 & 1.122 & 0.589
\\ 
& Sp-Df-p-end & 0.007 & 0.040 & 0.305 & 0.686 & 0.963 & 0.152 & 0.071 & 0.007 & 0.028 & 0.187 & 0.472 & 0.747 & 2.652 & 1.068
\\ 
& Sp-Df-fp-end & 0.013 & 0.081 & 0.489 & 0.864 & 0.995 & 0.092 & 0.051 & 0.012 & 0.057 & 0.332 & 0.738 & 0.924 & 1.275 & 0.659
\\ \bottomrule % \hline

    \end{tabular}
\caption{\label{tab:exp_ablation_ref_table} \textbf{KITTI model on Apollo dataset. The full table for rotation and translation error.} The set of models are trained in solely in KITTI dataset or ApolloScape dataset. }
\end{table*}

% \begin{table*}[h]
%     \scriptsize
%     \centering
%     \begin{tabular}{lllllllllllll}
%         \toprule
%         \multirow{2}{*} {KITTI dataset} & \multicolumn{6}{c}{Rotation (inlier ratio, error median)} & \multicolumn{6}{c}{Translation (inlier ratio, error median)} \\
%         \cmidrule(r){2-7} \cmidrule(r){8-13} \\
%         KITTI Models & 0.01 & 0.02 & 0.05 & 0.1 & 0.5 & Med. & 0.1 & 0.2 & 0.5 & 1.0 & 2.0 & Med. \\
%         \midrule
        
% Si-Ran & 0.017 & 0.078 & 0.433 & 0.818 & 0.997 & 0.056 & 0.020 & 0.085 & 0.372 & 0.727 & 0.899 & 0.639
% \\ \hline
% Sp-Ran & 0.001 & 0.004 & 0.048 & 0.189 & 0.815 & 0.217 & 0.003 & 0.014 & 0.077 & 0.222 & 0.481 & 2.103
% \\ \hline
% Si-Df-f & 0.028 & 0.143 & 0.645 & 0.938 & 0.998 & 0.041 & 0.032 & 0.137 & 0.517 & 0.812 & 0.914 & 0.484
% \\ \hline
% Si-Df-p & 0.028 & 0.125 & 0.579 & 0.901 & 0.995 & 0.044 & 0.025 & 0.119 & 0.485 & 0.787 & 0.903 & 0.513
% \\ \hline
% Si-Df-fp & 0.028 & 0.161 & 0.680 & 0.947 & 0.998 & 0.038 & 0.037 & 0.135 & 0.519 & 0.816 & 0.916 & 0.484
% \\ \hline
% Sp-Df-f & 0.005 & 0.034 & 0.263 & 0.633 & 0.997 & 0.078 & 0.009 & 0.048 & 0.258 & 0.579 & 0.830 & 0.846
% \\ \hline
% Sp-Df-p & 0.023 & 0.100 & 0.527 & 0.875 & 0.996 & 0.047 & 0.025 & 0.108 & 0.454 & 0.770 & 0.887 & 0.539
% \\ \hline
% Sp-Df-f-end & 0.023 & 0.144 & 0.614 & 0.915 & 0.998 & 0.042 & 0.033 & 0.114 & 0.511 & 0.800 & 0.905 & 0.489
% \\ \hline
% Sp-Df-p-end & 0.021 & 0.142 & 0.613 & 0.932 & 1.000 & 0.041 & 0.029 & 0.119 & 0.498 & 0.798 & 0.905 & 0.503
% \\ \hline
% Sp-Df-fp-end & 0.018 & 0.103 & 0.535 & 0.910 & 1.000 & 0.048 & 0.037 & 0.131 & 0.498 & 0.805 & 0.917 & 0.504
% \\ \hline
% % Sp-Df-fp-end-1 & 0.012 & 0.089 & 0.489 & 0.882 & 1.000 & 0.051 & 0.040 & 0.129 & 0.482 & 0.791 & 0.911 & 0.518
% % \\ \hline
% % Sp-Df-fp-end-2 & 0.021 & 0.099 & 0.505 & 0.889 & 1.000 & 0.050 & 0.027 & 0.111 & 0.474 & 0.793 & 0.916 & 0.527
% % \\ \hline
% % Sp-Df-fp-end-3 & 0.022 & 0.103 & 0.517 & 0.896 & 1.000 & 0.049 & 0.035 & 0.125 & 0.486 & 0.799 & 0.912 & 0.513
% % \\ \hline

% \bottomrule
%     \end{tabular}
% \caption{\label{tab:exp_ablation_ref_table} \textbf{KITTI model on KITTI dataset. The full table for rotation and translation error.} The set of models are trained in solely in KITTI dataset or ApolloScape dataset. }
% \end{table*}

% % Please add the following required packages to your document preamble:
% % % \usepackage{multirow}
% % \begin{table*}[]
% % \scriptsize
% % \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% % \hline
% % \multirow{3}{*}{} {\multirow{2}{*}{Models (KITTI)}} & \multicolumn{8}{l|}{KITTI dataset - Inlier ratio (w/i i degree)}       \\ \cline{2-9} 
% %                   {}                                & \multicolumn{4}{l|}{Rot.} & \multicolumn{4}{l|}{Trans} \\ \cline{2-9} 
% %                   & 0.02 & 0.1   & 1     & med.  & 0.1   & 1 & 2     & med.        \\ \hline
% % {[}0{]}            & &&&&&&&                     \\ \hline
% % {[}1{]}            & 0.007 & 0.252 & 0.966 & 0.177 & 0.003 & 0.234 & 0.483 & 2.050                     \\ \hline
% % {[}2{]}            & 0.126 & 0.942 & 0.999 & 0.043 & 0.022 & 0.751 & 0.857 & 0.562   \\ \hline
% % {[}3{]}            & 0.105 & 0.882 & 0.996 & 0.047 & 0.014 & 0.717 & 0.833 & 0.603 \\ \hline
% % {[}4{]}            & 0.144 & 0.939 & 1.000 & 0.042 & 0.022 & 0.737 & 0.850 & 0.567 \\ \hline
% % {[}5{]}            & 0.007 & 0.435 & 0.999 & 0.112 & 0.007 & 0.428 & 0.668 & 1.187 \\ \hline
% % {[}6{]}            & 0.033 & 0.647 & 0.998 & 0.078 & 0.012 & 0.547 & 0.766 & 0.898 \\ \hline
% % {[}7{]}            & 0.107 & 0.872 & 1.000 & 0.051 & 0.018 & 0.729 & 0.843 & 0.598 \\ \hline
% % {[}8{]}            & 0.091 & 0.772 & 0.998 & 0.060 & 0.027 & 0.680 & 0.831 & 0.685 \\ \hline
% % {[}9{]}            & 0.103 & 0.910 & 1.000 & 0.048 & 0.037 & 0.805 & 0.917 & 0.504   \\ \hline
% % \end{tabular}
% % \caption{\label{tab:exp_ablation_pipe} \textbf{Ablation study.} }
% % \end{table*}

